Dimension Mixer: Group Mixing of Input Dimensions for Efficient Function Approximation

The recent success of multiple neural architectures like CNNs, Transformers, and MLP-Mixers motivated us to look for similarities and differences between them. We found that these architectures can be interpreted through the lens of a general concept of dimension mixing. Research on coupling flows and the butterfly transform shows that partial and hierarchical signal mixing schemes are sufficient for efficient and expressive function approximation. In this work, we study group-wise sparse, non-linear, multi-layered and learnable mixing schemes of inputs and find that they are complementary to many standard neural architectures. Following our observations and drawing inspiration from the Fast Fourier Transform, we generalize Butterfly Structure to use non-linear mixer function allowing for MLP as mixing function called Butterfly MLP. We were also able to sparsely mix along sequence dimension for Transformer-based architectures called Butterfly Attention. Experiments on CIFAR and LRA datasets demonstrate that the proposed Non-Linear Butterfly Mixers are efficient and scale well when the host architectures are used as mixing function. Additionally, we propose Patch-Only MLP-Mixer for processing spatial 2D signals demonstrating a different dimension mixing strategy.

==> algs/alg_butterfly_mixer.tex <==
\begin{minted}[fontsize=\footnotesize,baselinestretch=1]{python}
# x : Input with shape [batch_size, input_dim].
# block_layers : Layers of block mixing function.
# fn_block : Block mixing function; is parallel non-linear mixer operating per block.
# block_dim : Radix or input size of a mixing function.  
# y : Output with same shape as Input x for simplicity.
y = x
for i, fn_block in enumerate(block_layers):
    stride = block_dim**i if ( block_dim**(i+1) <= input_dim ) else input_dim/block_dim
    y = y.view(-1, block_dim, stride).transpose(2, 1).view(batch_size, -1)
    y = fn_block(y)
    y = y.view(-1, stride, block_dim).transpose(2, 1).view(batch_size, -1)
return y
\end{minted}


==> tables/tab_solving_pathx_bkp0.tex <==
% p{0.25\textwidth}
\begin{tabularx}{\textwidth}{ >{\hsize=.1\hsize\linewidth=\hsize}X >{\hsize=0.9\hsize\linewidth=\hsize}X l c c c @{} }
\toprule
SN & Dataset & Samples & A & B & C \\
\midrule
1& Pathfinder32-contour-length-14 : Benchmark & \includegraphics[width=.6\textwidth,valign=M]{figures/pathX_intermediate/pf32_merge.png} & 69.17 & 68.53 & 74.86 \\
2& Pathfinder64-contour-length-9 : Benchmark & \includegraphics[width=.6\textwidth,valign=M]{figures/pathX_intermediate/pf64_merge.png} & 80.99 & 70.19 & 79.06 \\
3& PathX-cl14-nogap : We use parametrs similar to Path-X but reduce the number of distractors and gap (=1) between the dashes in the path. & $\includegraphics[width=.6\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_nogap.png}$ & 71.84 & 67.98 & 67.26\\
4& PathX-cl14-alpha0.0 : We increase the gap between dashes to be 2.     & \includegraphics[width=.6\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_alpha0.0.png} & 75.05 & 57.7 & 69.9\\
5& PathX-cl14-alpha0.75 : We increase the distractors and gap to be 2 or 3.  & \includegraphics[width=.6\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_alpha0.75.png} & 75.46 & 54.37 & 70.92 \\
6& PathX-cl14-alpha1.25 : We compare with pathfinder-X and try to reproduce the number of distractors & \includegraphics[width=.6\textwidth,valign=c]{figures/pathX_intermediate/pathX-cl14_alpha1.25.png} & 76.41 & 54.26 & 70.05 \\
7& PathX-contour-length-14 : Benchmark  & \includegraphics[width=.6\textwidth,valign=c]{figures/pathX_intermediate/pathX-curv_contour_length_14.png} & 76.72 & 53.6 & 54.04 \\
\bottomrule
\end{tabularx}


% \begin{tabularx}{ccc}
% text & \includegraphics[scale=0.25]{example-image} & text\\
% text & \includegraphics[align=c,scale=0.25]{example-image} & text\\
% text & \includegraphics[align=t,scale=0.25]{example-image} & text\\
% \end{tabularx}


==> tables/tab_solving_pathx_bkp1.tex <==
% p{0.25\textwidth}
% https://texdoc.org/serve/tabularx/0
\begin{tabularx}{\textwidth}{>{\hsize=0.3\hsize\linewidth=\hsize}X >{\hsize=0.6\hsize\linewidth=\hsize}Xlccc@{} }
\toprule
Dataset & Source & Samples & A & B & C \\
\midrule
Path32-cl-14 & LRA Benchmark & \includegraphics[width=.60\textwidth,valign=M]{figures/pathX_intermediate/pf32_merge.png} & 69.17 & 68.53 & 74.86 \\
Path64-cl-9 & LRA Benchmark & \includegraphics[width=.60\textwidth,valign=M]{figures/pathX_intermediate/pf64_merge.png} & 80.99 & 70.19 & 79.06 \\
PathX-cl14-nogap &Modified Path-X\newline distractors = 5 \newline gap  = 1& \includegraphics[width=.60\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_nogap.png} & 71.84 & 67.98 & 67.26\\
PathX-cl14-alpha0.0 & distractors = 5 \newline gap  = 2  & \includegraphics[width=.60\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_alpha0.0.png} & 75.05 & 57.7 & 69.9\\
PathX-cl14-alpha0.75 & distractors = 14\newline gap  = 2, 3  & \includegraphics[width=.60\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_alpha0.75.png} & 75.46 & 54.37 & 70.92 \\
PathX-cl14-alpha1.25 & distractors = 20 \newline gap  = 2, 3 & \includegraphics[width=.60\textwidth,valign=c]{figures/pathX_intermediate/pathX-cl14_alpha1.25.png} & 76.41 & 54.26 & 70.05 \\
PathX-cl-14 & LRA Benchmark  & \includegraphics[width=.60\textwidth,valign=c]{figures/pathX_intermediate/pathX-curv_contour_length_14.png} & 76.72 & 53.6 & 54.04 \\
\bottomrule
\end{tabularx}


% \begin{tabular}{@{}cccccclccc@{}}
% \toprule
% \rotatebox{90}{Image Size}&\rotatebox{90}{Contour Length}&\rotatebox{90}{Generated}&\rotatebox{90}{Num Distractors}&\rotatebox{90}{Paddle Gap}&\rotatebox{90}{Paddle Contrast}&Samples&A&B&C \\
% \midrule
% 32&14&\xmark&-&-&-&\includegraphics[width=.75\textwidth,valign=M]{figures/pathX_intermediate/pf32_merge.png}&69.17&68.53&74.86 \\
% 64&9&\xmark&-&-&-&\includegraphics[width=.75\textwidth,valign=M]{figures/pathX_intermediate/pf64_merge.png}&80.99&70.19&79.06 \\
% 128&14&\cmark&5&1&0.9&\includegraphics[width=.75\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_nogap.png}&71.84&67.98&67.26\\
% 128&14&\cmark&5&2&0.9& \includegraphics[width=.75\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_alpha0.0.png}&75.05&57.7&69.9\\
% 128&14&\cmark&14&2,3&0.8&\includegraphics[width=.75\textwidth,valign=M]{figures/pathX_intermediate/pathX-cl14_alpha0.75.png}&75.46&54.37&70.92 \\
% 128&14&\cmark&20&2,3&0.73&\includegraphics[width=.75\textwidth,valign=c]{figures/pathX_intermediate/pathX-cl14_alpha1.25.png}&76.41&54.26&70.05 \\
% 128&14&\xmark&-&-&-&\includegraphics[width=.75\textwidth,valign=c]{figures/pathX_intermediate/pathX-curv_contour_length_14.png}&76.72&53.6&54.04 \\
% \bottomrule
% \end{tabular}

==> tables/tab_sparse_approx.tex <==
\begin{tabular}{@{}lccccccc@{}}

\toprule 

\multirow{2.5}{*}{Size ($N$)}
& \multicolumn{5}{c}{Linear Butterfly} & \multicolumn{2}{c}{Low Rank Factorization} \\

\cmidrule(lr){2-6} \cmidrule(lr){7-8}

\textbf{}& 2 & $\sqrt{N}/2$ & $\sqrt{N}$ & Parallel (2) & Sequential (2) & Same Param. & $N/4$ \\

\midrule

\multirow{2}{*}{16}
& 0.171 \textcolor{brown}{0.254} & 0.171 \textcolor{brown}{0.254} & 0.136 \textcolor{brown}{0.230} & 1.2x10$^{-7}$ \textcolor{brown}{2.7x10$^{-4}$}  & 7.8x10$^{-4}$ \textcolor{brown}{0.019}  & 0.123 \textcolor{brown}{0.213} & 0.033 \textcolor{brown}{0.114} \\
& \textcolor{blue}{128} \textcolor{purple}{0.27} & \textcolor{blue}{128} \textcolor{purple}{0.27} & \textcolor{blue}{128} \textcolor{purple}{0.12}  & \textcolor{blue}{512} \textcolor{purple}{1.15}  & \textcolor{blue}{512} \textcolor{purple}{1.13}  & \textcolor{blue}{128} \textcolor{purple}{0.06} & \textcolor{blue}{256} \textcolor{purple}{0.05}   \\

\midrule

\multirow{2}{*}{64}
& 0.260 \textcolor{brown}{0.282} & 0.240 \textcolor{brown}{0.276} &  0.212 \textcolor{brown}{0.267} & 0.021 \textcolor{brown}{0.100} &  0.038 \textcolor{brown}{0.122} &  0.208 \textcolor{brown}{0.261} &  0.036 \textcolor{brown}{0.114} \\
& \textcolor{blue}{768} \textcolor{purple}{0.40} & \textcolor{blue}{768} \textcolor{purple}{0.18} & \textcolor{blue}{1024} \textcolor{purple}{0.12} & \textcolor{blue}{4608} \textcolor{purple}{2.48} & \textcolor{blue}{4608} \textcolor{purple}{2.45} & \textcolor{blue}{1024} \textcolor{purple}{0.06} & \textcolor{blue}{4096} \textcolor{purple}{0.05} \\

\midrule

\multirow{2}{*}{256}
& 0.305 \textcolor{brown}{0.288} & 0.278 \textcolor{brown}{0.284} & 0.265 \textcolor{brown}{0.282} & 0.136 \textcolor{brown}{0.223} & 0.141 \textcolor{brown}{0.223} & 0.263 \textcolor{brown}{0.280} & 0.035 \textcolor{brown}{0.113} \\
& \textcolor{blue}{4096} \textcolor{purple}{0.52} & \textcolor{blue}{6144} \textcolor{purple}{0.18} & \textcolor{blue}{8192} \textcolor{purple}{0.12} & \textcolor{blue}{32768} \textcolor{purple}{5.20} & \textcolor{blue}{32768}  \textcolor{purple}{4.27} & \textcolor{blue}{8192} \textcolor{purple}{0.07} & \textcolor{blue}{65536} \textcolor{purple}{0.06} \\

\midrule
 
\multirow{2}{*}{1024}
& 0.323 \textcolor{brown}{0.289} & 0.303 \textcolor{brown}{0.287} & 0.296 \textcolor{brown}{0.287} & 0.238 \textcolor{brown}{0.272} & 0.238 \textcolor{brown}{0.272} & 0.296 \textcolor{brown}{0.286} & 0.035 \textcolor{brown}{0.113} \\
& \textcolor{blue}{20.5K} \textcolor{purple}{0.63} & \textcolor{blue}{49.2K} \textcolor{purple}{0.18} & \textcolor{blue}{65.5K} \textcolor{purple}{0.36} & \textcolor{blue}{204.8K} \textcolor{purple}{41.17} & \textcolor{blue}{204.8K} \textcolor{purple}{23.14} & \textcolor{blue}{65.5K} \textcolor{purple}{0.06} & \textcolor{blue}{1.048M} \textcolor{purple}{0.06} \\

\midrule

\multirow{2}{*}{4096}
& 0.330 \textcolor{brown}{0.289} & 0.317 \textcolor{brown}{0.288} & 0.314 \textcolor{brown}{0.288} & --- & --- & 0.314 \textcolor{brown}{0.288} & 0.035 \textcolor{brown}{0.113} \\
& \textcolor{blue}{98.3K} \textcolor{purple}{20.55} & \textcolor{blue}{393.2K} \textcolor{purple}{0.18} & \textcolor{blue}{524.3K} \textcolor{purple}{4.93} & --- & --- & \textcolor{blue}{524.3K} \textcolor{purple}{0.07} & \textcolor{blue}{16.77M} \textcolor{purple}{0.32}\\

\bottomrule

\end{tabular}

